GIARPS High-resolution Observations of T Tauri stars (GHOsT). IV. Accretion properties of the Taurus-Auriga young association

In the framework of the GIARPS@TNG High-resolution Observations of T Tauri stars (GHOsT) project, we study the accretion properties of 37 Classical T Tauri Stars of the Taurus-Auriga star forming region (SFR) with the aim of characterizing their relation with the properties of the central star, of jets and disk winds, and of the global disk structure, in synergy with complementary ALMA millimiter observations. We derive stellar parameters, optical veiling, accretion luminosity ($\rm L_{acc}$) and mass accretion rate ($\rm \dot M_{acc}$) in a homogeneous and self-consistent way using high-resolution spectra acquired at the Telescopio Nazionale Galileo with the HARPS-N and GIANO spectrographs, and flux-calibrated based on contemporaneous low-resolution spectroscopic and photometric ancillary observations. The $\rm L_{acc}$-$\rm L_{\star}$, $\rm \dot{M}_{acc}$-$\rm M_{\star}$ and $\rm \dot{M}_{acc}$-$\rm M_{disk}$ relationships of the Taurus sample are provided and compared with those of the coeval SFRs of Lupus and Chamaeleon I. Our results demonstrate the potential of contemporaneous optical and near-infrared high-resolution spectroscopy to simultaneously provide precise measurements of stellar and accretion/wind properties of young stars.

==> Tables/JournalOfObservationsAndSourcesParameters_old.tex <==
\begin{table*}
\small
\center
\caption{\label{tab:sources_param} Gaiai EDR3 distances and stellar properties derived in this work.}
\begin{tabular}{lclcccccccc}
\hline
\hline
Source    & Obs Date   & $\rm T_{eff}$ $\rm (\pm err)$ & r600 & SpT & $\rm A_v (\pm err) $ & $\rm L_\star$ & $\rm R_\star$ & $\rm M_\star$ & $\rm log \bigl\langle L_{acc} \bigr\rangle$ & $\rm log \dot M_{acc}$     \\
          &        & [K] & &  & [mag] & [$\rm L{\odot}$] & [$\rm R_{\odot}$] &  [$\rm M_{\odot}$]& [$\rm L_{\odot}$]  & [$\rm M_{\odot}$ $\rm yr^{-1}$]         \\
\hline
\multicolumn{11}{c}{Accreating sources} \\
\hline
 BP Tau          & 26 Gen 2020 & 4198 (105)	 & 0.5    & K5  & 0.30 (0.10) & 0.23 & 0.91 & 0.79 & -1.29 (0.07) & -8.63 \\
 CI Tau          & 09 Dec 2018 & 4559 (114)  & 0.8    & K4  & 2.30 (0.20) & 0.76 & 1.40 & 1.18 & -0.13 (0.06) & -7.46 \\      
 CQ Tau          & 13 Nov 2017$\rm ^{(e)}$  &  6823 (136) & 0.0 & F4 & 0.50 & < 15.13 & < 2.75 & < 1.99 & < -0.42 & < -7.70   \\
 CW Tau          & 20 Dec 2015 & -	         & -      & -   & -           & -    & -    & -    & -            & -     \\
                 & 08 Dec 2018 & 4584 (95)	 & 2.0    & K0  & 3.50 (0.20) & 0.36 & 0.85 & 0.90 & -0.12 (0.07) & -7.54 \\
 CY Tau          & 13 Dec 2020 & 3559 (88)   & 0.0    & M2  & 0.00 (0.10) & 0.12 & 0.91 & 0.36 & -2.00 (0.07) & -9.00 \\
 DD Tau          & 19 Dec 2015 & -	         & -      & -   & -           & -    & -    & -    & -            & -     \\
 DE Tau          & 24 Oct 2020 & 3499 (57)   & 0.1    & M2V & 0.00 (0.10) & 0.33 & 1.56 & 0.36 & -1.46 (0.08) & -8.22 \\  
 DF Tau          & 20 Dec 2015 & -	         & -      & -   & -           & -    & -    & -    & -            & -     \\ 
                 & 08 Dec 2018 & 3565 (92)	 & 0.7    & M2  & 0.00 (0.20) & 0.29 & 1.41 & 0.38 & -0.74 (0.07) &  -7.57 \\
 DG Tau          & 19 Dec 2015 & -           & -      & -   & -           & -    & -    & -    & -            & -     \\
                 & 29 Oct 2017$\rm ^{(a)}$   & 4004 (153) & 1.5 & K7 & 1.50 & 0.44 & 1.38 & 0.70 & -0.25 (0.18) & -7.35 \\
 DH Tau          & 02 Nov 2019 &  3631 (87)	 & 1.0    & M1  & 0.60        & 0.20 & 1.13 & 0.41 & -1.50 (0.07) & -8.46 \\
 DK Tau          & 08 Dec 2018 & 4270 (106)	 & 0.2    & K5  & 0.80 (0.20) & 0.41 & 1.17 & 0.99 & -1.62 (0.07) & -8.95 \\
 DL Tau          & 20 Dec 2015 & -           & -      & -   & -           & -    & -    & -    & -            & -     \\
                 & 29 Oct 2017$\rm ^{(a)}$   & 4188 (100) & 1.2 & K5 & 1.50 & 0.40 & 1.20 & 0.90 & -0.35 (0.18) & -7.62\\
 DN Tau          & 01 Nov 2019 & 4236 (67)	 & 0.0    & K5  & 0.80 (0.20) & 0.43 & 1.22 & 0.98 & -2.07 (0.09) &  -9.37 \\
 DO Tau          & 19 Dec 2015 & -	         & -      & -   & -           & -    & -    & -    & -            & -      \\
                 & 13 Nov 2017$\rm ^{(a)}$ & 3694 (104) & 1.0 & M1 & 1.40 & 0.42 & 1.58 & 0.50 & -0.84 (0.16) & -7.73 \\
                 & 26 Gen 2020 & 3630 (132)	 & 1.2    & M1  & 1.40 (0.20) & 0.27 & 1.31 & 0.42 & -1.03 (0.07) & -7.94 \\
 DQ Tau          & 02 Nov 2019 & 4044 (103)	 & 0.3    & K7  & 1.50 (0.20) & 0.71 & 1.72 & 0.75 & -0.88 (0.07) & -7.92 \\
 DR Tau          & 25 Gen 2020 & 4447 (161)	 & 3.5    & K4  & 1.20 (0.20) & 0.29 & 0.91 & 0.83 & -0.56 (0.08) & -7.92 \\
 DS Tau	         & 01 Nov 2019 & 4244 (130)	 & 1.0    & K5  & 0.40 (0.10) & 0.21 & 0.85 & 0.79 & -1.46 (0.07) & -8.83 \\
 FT Tau          & 25 Gen 2020 & 3407 (73)	 & 1.5    & M3  & 0.60 (0.20) & 0.03 & 0.50 & 0.24 & -1.92 (0.09) & -9.00 \\
 GG Tau          & 09 Dec 2018 & 4168 (121)	 & 0.2    & K6  & 1.40 (0.20) & 0.67 & 1.57 & 0.91 & -0.76 (0.08 )& -7.92 \\
 GH Tau          & 25 Gen 2020 & 3632 (67)	 & 0.2    & M1  & 0.80 (0.20) & 0.38 & 1.56 & 0.42 & -2.23 (0.09) & -9.06 \\
 GI Tau          & 26 Gen 2020 & 3957 (140)	 & 0.7    & K7  & 2.10 (0.20) & 0.20 & 0.95 & 0.74 & -1.27 (0.07) & -8.56 \\
 GK Tau          & 02 Nov 2019 & 4439 (89)	 & 0.2    & K4  & 1.90 (0.10) & 0.82 & 1.53 & 1.19 & -1.39 (0.10) & -8.68 \\
 GM Aur          & 09 Dec 2018 & 4564 (76)	 & 0.0    & K3  & 1.30 (0.20) & 1.16 & 1.72 & 1.19 & -1.04 (0.09) & -8.28 \\
 HL Tau          & 24 Nov 2016 &  	         &        &     &             &      &      &      & & \\
 HN Tau          & 19 Dec 2015 & -	         & -      & -   & -           & -    & -    & -    & -            & -     \\
                 & 29 Oct 2017$\rm ^{(e)}$ & 4617 (97) & 0.8 & K4 & 1.25 & 2.63 & 2.57 & 1.58 & -0.12 (0.23) & -7.19 \\
 HQ Tau          & 01 Nov 2019 & 5182 (87)	 & 0.0    & G8  & 3.70 (0.10)     & 5.51 & 2.91 & 2.09  & -1.23 (0.14) & -8.49  \\
 IP Tau          & 09 Dec 2018 & 4258 (97)	 & 0.1    & K5  & 0.90 (0.20)     & 0.25 & 0.92 & 0.79 & -2.05 (0.10) & -9.38 \\
 IQ Tau          & 02 Nov 2019 & 3811 (65)$\rm ^{(b)}$  & 1.5$\rm ^{(c)}$ & M0     & 1.60 (0.10) & 0.14 & 0.86 & 0.55 & -1.40 (0.08) & -8.61\\
 LkCa 15         & 14 Dec 2020  & 4588 (73)  & 0.1    & K4  & 0.90 (0.20)  & 0.57  & 1.19 & 1.07  & -1.89 (0.09) & -9.24 \\
 MWC480          & 01 Nov 2019  & 8500     	 & 0.0    & F0   & 0.00 (0.10) & 13.49 & 1.69 & 1.90 & -0.19 (0.12) & -7.64 \\
 RW Aur A        & 13 Nov 2017$\rm ^{(a)}$   & 4870 & 1.2 & K0 & 1.00 & 1.64 & 1.80 & 1.50 & +0.39 (0.30) & -6.93 \\
 RY Tau          & 20 Dec 2015 & -           & -      & -   & -           & -    & -    & -    & - & -  \\
                 & 13 Nov 2017$\rm ^{(a)}$   & 5856 (151) & 0.0 & G1 & 2.25 & 8.87 & 2.89 & 1.80 & -0.38 (0.15) & -7.57 \\
 SU Aur          & 24 Oct 2020 & 5414 (171)  & 0.0    & G5III & 0.90 (0.10) & 8.66 & 3.34 & 2.21 & -0.54 (0.10) & -7.76 \\
 UX Tau          & 26 Gen 2020 & 5243 (73)	 & 0.0    & G8  & 1.20 (0.10) & 1.62 & 1.54 & 1.30 & -1.26 (0.16) & -8.59 \\
 UY Aur          & 08 Dec 2018 & 4086 (138)	 & 0.4    & K7  & 0.70 (0.20) & 0.41 & 1.28 & 0.81 & -1.18 (0.07) & -8.38 \\
 UZ Tau E        & 09 Dec 2018 & 3609 (112)	 & 0.7    & M2  & 0.70 (0.20) & 0.34 & 1.49 & 0.41 & -1.27 (0.07) & -8.11 \\
 V409 Tau        & 26 Gen 2020 & 3649 (106)	 & 0.5    & M1  & 0.30 (0.20) & 0.18 & 1.06 & 0.42 & -2.64 (0.13) & -9.64 \\
 V807 Tau$\rm ^{(d)}$ & 24 Oct 2020 & 4562 (79)   & 0.2    & K4V & 1.30 (0.20) & 1.69 & 2.08 & 1.49 & -0.91 (0.09) & -8.16 \\
 V836 Tau        & 02 Nov 2019 & 4444 (86)	 & 0.1    & K5  & 0.80 (0.20)  & 0.28     & 0.89  & 0.84 & -2.15 (0.09) & -9.52 \\
                 & 26 Gen 2020 & 4389 (100)  & 0.1    & K5  & 0.70 (0.20)  & 0.24     & 0.85   & 0.79  & -2.06 (0.09) & -9.43 \\
 XZ Tau          & 14 Mar 2017 & 	         &        &     &             &      &      &      & & \\
\hline
\multicolumn{11}{c}{Class III / debris sources} \\
\hline
DI Tau	        & 13 Dec 2020 & 4022 (85)   & 0.0    & M0  & 0.50 (0.10) & 0.40 & 1.30  & 0.75 &  &  \\
IW Tau			& 13 Dec 2020  & 4271 (75)  & 0.0    & K7  & 0.60 (0.20) & 0.50  & 1.29 & 1.00 &  &   \\
LkCa 4		    & 13 Dec 2020  & 4085 (139) & 0.0    & K7  & 0.20 (0.10) & 0.31  & 1.11 & 0.80 &  &  \\ 
LkCa 21		    & 13 Dec 2020  & 3682 (116) & 0.0    & M1.5 & 0.60 (0.20) & 0.23 & 1.18 & 0.45 &  &  \\
V819 Tau    	& 14 Dec 2020 & 4539 (72)   & 0.0    & K4  & 1.90 (0.20) & 0.64 & 1.30 & 1.03 &  &  \\
V827 Tau        & 13 Dec 2020 & 4397 (105)  & 0.1    & K7  & 0.10 (0.20)  & 0.37     & 1.05  & 0.94 & &  \\
V1070 Tau       & 13 Dec 2020 & 4399 (108)  & 0.0    & K5    & 0.60 (0.20) & 0.42 & 1.12 & 1.00 &  &  \\
V1098 Tau       & 24 Oct 2020 & 3837 (138)  & 0.1    & M1.0V & 0.00 (0.20) & 0.53 & 1.65 & 0.56 &  &  \\
V1115 Tau       & 14 Dec 2020 & 4565 (73)   & 0.0    & K4  & 0.40 (0.10) & 0.59 & 1.23 & 1.07 &  &  \\
\hline\end{tabular}	
\begin{quotation}
\textbf{Notes.} 
$\rm ^{(a)}$ Parameters derived in \citet{Alcala2021}. $\rm ^{(b)}$ Value taken from APOGEE-2 DR16 \citep{Jonsson2020}. $\rm ^{(c)}$ Estimated using GES and PALLA models. $\rm ^{(d)}$ Triple system: $\rm L_{\star}$, $\rm R_{\star}$ and $\rm M_{\star}$ taken from \citet{Schaefer2012} and scaled with the new Gaia DR3 distance. $\rm ^{(e)}$ Subluminous YSO: the reported values are corrected for obscuration effects (See Section 4.3.1 of \citet{Alcala2021}).
\end{quotation}
\end{table*} 

